Scanning For Dark Matter Subhalos in Hubble Space Telescope Imaging of 54 Strong Lenses

The cold dark matter (DM) model predicts that every galaxy contains thousands of DM subhalos; almost all other DM models include a physical process that smooths away the subhalos. The subhalos are invisible, but could be detected via strong gravitational lensing, if they lie on the line of sight to a multiply-imaged background source, and perturb its apparent shape. We present a predominantly automated strong lens analysis framework, and scan for DM subhalos in Hubble Space Telescope imaging of 54 strong lenses. We identify five DM subhalo candidates, including two especially compelling candidates (one previously known in SLACS0946+1006) where a subhalo is favoured after all of our tests for systematics. We find that the detectability of subhalos depends upon the assumed parametric form for the lens galaxy's mass distribution, especially its degree of azimuthal freedom. Using separate components for dark matter and stellar mass reveals two DM subhalo candidates and removes four false-positives compared to the single power-law mass model that is common in the literature. We identify 45 lenses without substructures, the number of which is key to statistical tests able to rule out models of e.g. warm or self-interacting DM. Our full analysis results are available at https://github.com/Jammy2211/autolens_subhalo.

==> A_Table.tex <==
\section{Mass Model Parameters}\label{TableApp}

\begin{table*}
\tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{ l | l | l | l l l l l l l } 
\multicolumn{1}{p{1.8cm}|}{\centering \textbf{Model}} 
& \multicolumn{1}{p{1.1cm}|}{\centering \textbf{Component}} 
& \multicolumn{1}{p{1.5cm}}{\textbf{Parameters}} 
& \multicolumn{1}{p{1.5cm}}{} 
& \multicolumn{1}{p{1.5cm}}{} 
\\ \hline
& & & & & \\[-4pt]
\textbf{S\'ersic} & Light + Mass & ($x$, $y$): centre $(\arcsec)$ & ($\epsilon_{\rm 1}$, $\epsilon_{\rm 2}$): elliptical components  \\[2pt]
               & (Stellar)  & $I$: Intensity & $R$: Effective Radius $(\arcsec)$ & $n$: S\'ersic index\\[2pt]
               & & $\Psi$: Mass-to-Light Ratio (e$^{\rm -\,1}$\,s$^{\rm -1}$) & $\Gamma$: Radial Gradient of $\Psi$ & \\[2pt]
               \hline
& & & & & & \\[-4pt]
\textbf{Elliptical} & Lens Mass & ($x^{\rm mass}$, $y^{\rm mass}$): centre $(\arcsec)$ & ($\epsilon^{\rm mass}_{\rm 1}$, $\epsilon^{\rm mass}_{\rm 2}$): elliptical components  \\[2pt]
\textbf{Power-Law (PL)} & (Total)  & $\theta^{\rm mass}_{\rm  E}$: Einstein Radius $(\arcsec)$ & $\gamma^{\rm mass}$: density slope \\[2pt]
& & & & & & \\[-4pt]
\hline
\textbf{Singular Isothermal} & Lens Mass  & ($x^{\rm mass}$, $y^{\rm mass}$): centre & ($\epsilon^{\rm mass}_{\rm 1}$, $\epsilon^{\rm mass}_{\rm 2}$): elliptical components  \\[2pt]
\textbf{Ellipsoid} (SIE)   & (Total) &$\theta^{\rm mass}_{\rm  E}$: Einstein Radius \\[2pt]
\hline
& & & & & \\[-4pt]
\textbf{Singular Isothermal} & Line Of & ($x^{\rm mass}$, $y^{\rm mass}$): centre &  \\[2pt]
\textbf{Sphere} (SIS)   & Sight Galaxies     &$\theta^{\rm mass}_{\rm  E}$: Einstein Radius \\[2pt]
\hline
& & & & & & \\[-4pt]
\textbf{Broken} & Lens Mass & ($x^{\rm mass}$, $y^{\rm mass}$): centre $(\arcsec)$ & ($\epsilon^{\rm mass}_{\rm 1}$, $\epsilon^{\rm mass}_{\rm 2}$): elliptical components  \\[2pt]
 \textbf{Power-Law (BPL)} & (Total) & $\kappa^{\rm mass}_{\rm E}$: Convergence Break Radius $(\arcsec)$ & $t^{\rm mass}_{\rm 1}$: inner density slope \\[2pt]
\hline
& & & & & & \\[-4pt]
\textbf{Power-Law} & Lens Mass & ($x^{\rm mass}$, $y^{\rm mass}$): centre $(\arcsec)$ & ($\epsilon^{\rm mass}_{\rm 1}$, $\epsilon^{\rm mass}_{\rm 2}$): elliptical components &    \\[2pt]
\textbf{With Multipoles} & (Total)  & $\theta^{\rm mass}_{\rm  E}$: Einstein Radius $(\arcsec)$ & $\gamma^{\rm mass}$: density slope \\[2pt]
 & & $(\gamma_{\rm 1}^{\rm mp},\ \gamma_{\rm 2}^{\rm mp})$: multipole components   \\[2pt]
\hline
& & & & & \\[-4pt]
\textbf{Elliptical NFW} & Lens Mass & ($x^{\rm dark}$, $y^{\rm dark}$): centre $(\arcsec)$ & ($\gamma_{\rm 1}^{\rm dark}$, $\gamma_{\rm 2}^{\rm dark}$): elliptical components  & \\[2pt]
            & (Dark)  & $M_{\rm 200}^{\rm dark}$: Mass at 200 (M$_{\rm \odot}$) & \\[2pt]
\hline
\textbf{Spherical NFW} & DM Subhalo & ($x^{\rm sub}$, $y^{\rm sub}$): profile center &  $M_{\rm 200}^{\rm sub}$: Enclosed mass at $r_{200}$ & \\[2pt]
\hline
& & & & & \\[-4pt]
\textbf{Shear} & Line-of-sight & ($\gamma_{1}^{\rm ext}$, $\gamma_{2}^{\rm ext}$): elliptical components & \\[2pt] 
\end{tabular}
}
\caption{The light and mass profiles used in this work. Column 1 gives the model name and abbreviation in brackets. Column 2 gives whether it models the lens's light, mass, subhalo or line-of-sight. For mass models, the brackets also indicate if it models the total mass (stellar and dark) or just the stellar or dark matter. Column 3 onwards gives the model's associated parameters.}
\label{table:SimModels}
\end{table*}

\cref{table:SimModels} summarizes all of the mass models fitted in this work, including what component of mass they represent and their free parameters.

==> figures/bells/residuals.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0755+3445.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0918+5104.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1226+5457.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0029+2544.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0201+3228.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ2342-0120.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1110+3649.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1201+4743.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0856+2010.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0113+0250.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ2228+1205.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1110+2808.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0742+3341.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1141+2216.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ0237-0641.pdf}
\includegraphics[width=0.16\textwidth]{Data/Bells/Resi/SDSSJ1116+0915.pdf}
\caption{The subhalo scanning results of the BELLS-GALLERY strong lens sample. Each scan uses a $5 \times 5$ grid of {\tt dynesty} non-linear searches fitting a power-law plus shear model with a subhalo whose (x,y) coordinates are confined to a 2D grid-cell via uniform priors. Fits are shown in descending order of highest Bayesian evidence increase $\Delta\,\mathrm{ln}\,\epsilon_{\rm sub}$. The background images show the lens subtracted data, where the lens subtraction uses a double Sersic fit.}
\label{figure:ResiSBells}
\end{figure*}

==> figures/criteria.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.24\textwidth]{Data/Criteria/slacs1420+6019_base.pdf}
\includegraphics[width=0.24\textwidth]{Data/Criteria/slacs1420+6019_delaunay.pdf}
\includegraphics[width=0.24\textwidth]{Data/Criteria/slacs1630+4520_base.pdf}
\includegraphics[width=0.24\textwidth]{Data/Criteria/slacs1630+4520_delaunay.pdf}
\caption{
Subhalo scanning results for two lenses which illustrate edge-cases of our subhalo candidate criteria. Each scan uses a $5 \times 5$ grid of {\tt dynesty} non-linear searches fitting a power-law plus shear model with a subhalo whose (x,y) coordinates are confined to a 2D grid-cell via uniform priors. Results for the Voronoi and Delaunay pixelizations are shown. For SLACS1420+6019 (left panels) only the Voronoi pixelization gives a log likelihood increase above the threshold $\Delta\,\mathrm{ln}\,\mathcal{L} > 10$. However, the Delaunay gives an log likelihood below $10$ in the same image-plane cell. Owing to their consistency we consider this a candidate subhalo detection, even though one pixelization is below the threshold $\Delta\,\mathrm{ln}\,\mathcal{L} > 10$. For SLACS1630+4520 both pixelizations infer $\Delta\,\mathrm{ln}\,\mathcal{L} > 10$, however the log likelihood increases are in different regions of the image-plane, meaning this is not considered a candidate subhalo detection.
}
\label{figure:Criteria}
\end{figure*}

==> figures/fp/mass_0.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.24\textwidth]{Data/FP/Mass/slacs0029-0055_gui_mask_image_squared.png}
\includegraphics[width=0.24\textwidth]{Data/FP/Mass/slacs0029-0055_gui_mask_model_image.pdf}
\includegraphics[width=0.24\textwidth]{Data/FP/Mass/slacs0029-0055_decomp_model_image.pdf}
\includegraphics[width=0.24\textwidth]{Data/FP/Mass/slacs0029-0055.pdf}
\caption{
The lens SLACS0029-0055, which illustrates how making the mass model more complex can lead one to favour a DM subhalo when a simpler mass model did not. The left panel shows the observed image, which includes a red square highlighting a feature in the lensed source's appearance. The left-centre panel shows a PL plus shear (without a DM subhalo) model-image, which does not reconstruct the lensed source feature shown in the red square. This model does not go on to favour a DM subhalo $\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm SO} = 4.59$. The right-centre panel shows the decomposed mass model (without a DM subhalo) model-image, which reconstructs the lensed source feature shown in the red square. This model goes on to favour a DM subhalo $\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm Decomp} = 21.52$. The right panel shows the subhalo scanning map using the decomposed model, where models including a DM subhalo produce a log likelihood increase around the lensed source feature. The inferred DM subhalo mass at $3\sigma$ confidence is $\mathrm{log}_{10}M^{\rm sub}_{\rm 200} = 1.09^{+0.42}_{-0.278} \times 10^{10}$M$_{\rm \odot}$ 
}
\label{figure:FPMass1}
\end{figure*}

==> figures/simulations/mass.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_0_subhalo_mass_105.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_0_subhalo_mass_100.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_0_subhalo_mass_95.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_0_no_subhalo.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_2_subhalo_mass_105.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_2_subhalo_mass_100.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_2_subhalo_mass_95.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_slacs_lens_2_no_subhalo.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_bells_lens_0_subhalo_mass_105.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_bells_lens_0_subhalo_mass_100.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_bells_lens_0_subhalo_mass_95.pdf}
\includegraphics[width=0.23\textwidth]{Data/SimFit/Mass/subhalo_delaunay_bells_lens_0_no_subhalo.pdf}
\caption{The subhalo masses inferred by the subhalo scan for every simulated lens. Each panel shows a $5 \times 5$ grid of {\tt dynesty} non-linear searches where the yellow overlay shows the subhalo mass. The (y,x) coordinates of each subhalo are confined to the 2D grid-cell via uniform priors and the inferred values are shown by black crosses. The input subhalo mass decreases from left to right and different lenses are shown across the rows. The source is modeled using a brightness based Delaunay pixelization. The subhalo location is marked with a black cross.}
\label{figure:SimMass}
\end{figure*}

==> figures/slacs/residuals.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs2341+0000.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0946+1006.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1432+6317.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0959+0410.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0728+3835.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1430+4105.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1250+0523.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1205+4910.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs2303+1422.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1143-0144.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0936+0913.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0252+0039.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1213+6708.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1630+4520.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1420+6019.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1032+5322.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1020+1122.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0737+3216.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0029-0055.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0330-0020.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1402+6321.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0008-0004.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0903+4116.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1627-0053.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1451-0239.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1525+3327.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs2238-0754.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1029+0420.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0216-0813.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0157-0056.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0912+0029.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs2300+0022.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1142+1001.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1218+0830.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs1023+4230.pdf}
\includegraphics[width=0.16\textwidth]{Data/Slacs/Resi/slacs0822+2652.pdf}
\caption{The subhalo scanning results of the SLACS strong lens sample. Each scan uses a $5 \times 5$ grid of {\tt dynesty} non-linear searches fitting a power-law plus shear model with a subhalo whose (x,y) coordinates are confined to a 2D grid-cell via uniform priors. Fits are shown in descending order of highest Bayesian evidence increase. The background images show the lens subtracted data, where the lens subtraction uses a double Sersic fit.}
\label{figure:ResiSlacs}
\end{figure*}

==> tables/mass_anti_fp.tex <==
\begin{table}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{ l | l | l | l | l} 
\multicolumn{1}{p{1.5cm}|}{Lens Name} 
& \multicolumn{1}{p{1.4cm}|}{Broken Power-Law} 
& \multicolumn{1}{p{1.4cm}|}{Power-Law with Multipoles} 
& \multicolumn{1}{p{1.4cm}|}{Decomposed} 
\\ \hline
SLACS1432+6317 & & 28.48 & \\[2pt]
SLACS0029-0055 & 10.93 & & 23.59 \\[2pt]
SLACS1143-0144 & & & 0.22 \\[2pt]
SLACS1029+0420 & & & 8.41 \\[2pt]
SLACS1205+4910 & & & 3.80 \\[2pt]
SLACS0252+0039 & & -9.58 &\\[2pt] 
SLACS0330-0020 & & -0.35 &\\[2pt]
SLACS1142+1001 & & & 8.62 \\[2pt]
SLACS2238-0754 & & -9.61 & \\[2pt]
SLACS0728+3835 & & -16.62 & \\[2pt]
\end{tabular}
\end{adjustbox}
\caption{
\red{There are 10 lenses where the PL mass model disfavoured a DM subhalo but at least one of the three more complex mass models (BPL, PL with multipoles, decomposed mass model) did. This table shows the inferred increase of Bayesian evidence $\Delta\,\mathrm{ln}\,\mathcal{Z}$ for these lenses in the \textbf{SH}$^3$ stage of the SLaM pipeline which fits each mass model with a DM subhalo. Values in columns 2, 3 and 4 are $\Delta\,\mathrm{ln}\,\mathcal{Z}$ inferred for the complex mass model (with subhalo) minus $\Delta\,\mathrm{ln}\,\mathcal{Z}$ inferred for the simpler PL (with subhalo). Values of $\Delta\,\mathrm{ln}\,\mathcal{Z} > 10$ indicate that the more complex mass model with a subhalo is favoured over the PL with a subhalo, which is only the case for 2 out of 10 lenses.}
}
\label{table:MassAntiFPPL}
\end{table}


==> tables/projections.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{ l | l | l | l | l } 
\multicolumn{1}{p{2.0cm}|}{Study} 
& \multicolumn{1}{p{2.5cm}|}{$z_{\rm lens}$}  
& \multicolumn{1}{p{2.0cm}|}{$z_{\rm src}$}  
& \multicolumn{1}{p{2.5cm}|}{$M^{\rm sub}_{\rm 200}$ range [\,M$_{\rm \odot}$]}  
& \multicolumn{1}{p{4.0cm}|}{Expected detections per lens (upper limit)}  
\\ \hline
Amorisco2021 & 0.2 & 0.6 & $10^{\rm 10-11}$ & 0.025 \\[2pt]
Amorisco2021 & 0.5 & 1.0 & $10^{\rm 10-11}$ & 0.1 \\[2pt]
He2022       & 0.2 & 1.0 & $10^{\rm 10-11}$ & 0.1 \\[2pt]
He2022       & 0.5 & 1.0 & $10^{\rm 10-11}$ & 0.3 \\[2pt]
\end{tabular}
\caption{The expected number of DM subhalo detections between certain mass ranges for lenses at different redshifts. As discussed in section \ref{DMExpect}, numbers are derived from the sensitivity mapping performed by \citet{Amorsico2021} and \cite5{He2022}. These studies both assume parametric Sersic sources, which as discussed in appendix \ref{SourceModel} make subhalos more detectable. The expected number of detections is an upper limit. Column 1 lists which study numbers are quoted from. Columns 2 and 3 show the assumed lens and source redshifts. Column 4 shows the subhalo mass range of which this prediction is made. Column 5 gives an upper limit on the expected number of detections per lens.}
\label{table:DetectExpect}
\end{table*}

==> tables/simulations/reg.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{
\begin{tabular}{ l | l | l | l | l | l | l | l | l } 
\multicolumn{1}{p{1.3cm}|}{Lens Name} 
& \multicolumn{1}{p{1.5cm}|}{Subhalo Mass}  
& \multicolumn{1}{p{1.5cm}|}{$\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm Vor}$}  

\\ \hline

 $\mathrm{Lens}_{1}$ & No Subhalo  & 1.7 & -2.1 & -1.11   & -0.18  \\[2pt]
 $\mathrm{Lens}_{1}$ & $10^{9.5}M_{\odot}$  & \textbf{17.67} & \textbf{16.75} & \textbf{28.26}   & 3.35  \\[2pt]
 $\mathrm{Lens}_{1}$ & $10^{10.0}M_{\odot}$  & \textbf{39.89} & \textbf{33.24} & \textbf{33.13}   & \textbf{33.78}  \\[2pt]
 $\mathrm{Lens}_{1}$ & $10^{10.5}M_{\odot}$  & \textbf{186.58} & \textbf{177.6} & \textbf{202.16}   & \textbf{119.8}  \\[2pt]
 $\mathrm{Lens}_{2}$ & No Subhalo  & 0.45 & -0.22 & \textbf{13.35}   & -0.19  \\[2pt]
 $\mathrm{Lens}_{2}$ & $10^{9.5}M_{\odot}$  & 3.71 & 1.28 & \textbf{17.52}   & 3.56  \\[2pt]
 $\mathrm{Lens}_{2}$ & $10^{10.0}M_{\odot}$  & 7.57 & \textbf{12.25} & 3.87   & 5.05  \\[2pt]
 $\mathrm{Lens}_{2}$ & $10^{10.5}M_{\odot}$  & \textbf{15.3} & \textbf{56.05} & \textbf{14.25}   & \textbf{16.95}  \\[2pt]
 $\mathrm{Lens}_{3}$ & No Subhalo  & 4.62 & -1.39 & -6.14   & 0.06  \\[2pt]
 $\mathrm{Lens}_{3}$ & $10^{9.5}M_{\odot}$  & \textbf{33.75} & \textbf{38.01} & \textbf{37.86}   & \textbf{13.51}  \\[2pt]
 $\mathrm{Lens}_{3}$ & $10^{10.0}M_{\odot}$  & \textbf{108.11} & \textbf{107.06} & \textbf{123.86}   & \textbf{57.36}  \\[2pt]
 $\mathrm{Lens}_{3}$ & $10^{10.5}M_{\odot}$  & \textbf{638.2} & \textbf{531.53} & \textbf{595.63}   & \textbf{274.93}  \\[2pt]
 $\mathrm{Lens}_{4}$ & No Subhalo  & 2.34 & -1.1 & 3.93   & -0.08  \\[2pt]
 $\mathrm{Lens}_{4}$ & $10^{9.5}M_{\odot}$  & 3.61 & \textbf{12.93} & \textbf{32.49}   & 0.96  \\[2pt]
 $\mathrm{Lens}_{4}$ & $10^{10.0}M_{\odot}$  & \textbf{18.24} & \textbf{29.02} & \textbf{10.9}   & \textbf{10.8}  \\[2pt]
 $\mathrm{Lens}_{4}$ & $10^{10.5}M_{\odot}$  & \textbf{89.54} & \textbf{111.36} & \textbf{105.94}   & \textbf{70.11}  \\[2pt]


\end{tabular}
}
\caption{
The highest log likelihood increases $\Delta\,\mathrm{ln}\,\mathcal{L}$ of the subhalo scanning results for fits to the simulated strong lens sample, where log likelihood increases are computed compared to the lens model fitted previously without a subhalo. All mass models assume a PL plus shear and a lens light subtraction consisting of two Sersic profiles. Results for the following four source reconstructions and masking schemes are shown: (i) Voronoi source with $3.5"$ circular mask ($\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm Vor}$); (ii) Delaunay source with $3.5"$ circular mask ($\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm Del}$); (iii) Voronoi source with source-only mask ($\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm VorSO}$) and; (iv) Delaunay source with source-only mask ($\Delta\,\mathrm{ln}\,\mathcal{L}^{\rm DelSO}$). Errors quoted on $x^{\rm sub}$, $y^{\rm sub}$ and $\log_{10}[M^{\rm sub}_{\rm 200}$\,/\,M$_{\rm \odot}]$ are at $3\sigma$ confidence. The true input subhalo coordinates $(x^{\rm sub}$,\,$y^{\rm sub})$ for each lens are: $\mathrm{Lens}_{1} = (0.3,\,1.9)$, $\mathrm{Lens}_{2} = (0.5,\,1.34)$, $\mathrm{Lens}_{3} = (0.3,\,1.9)$ and $\mathrm{Lens}_{4} = (-1.25,\,0.6)$.
}
\label{table:DetectSim}
\end{table*}

